ExtractBench Pro: The Long Tail of Document Extraction

We present ExtractBench Pro, a schema-guided document extraction benchmark that tests six challenging modes of extraction underrepresented in existing datasets. It is created following a framework for synthetic document generation, in which deterministic document generators assemble challenging components into documents that are designed to be difficult at a level calibrated for frontier systems. We synthesize 100 realistic documents spanning a diverse range of styles. On this data, we evaluate ten coding agents and eight extraction API configurations for accuracy, grounding, and their ability to perfectly extract documents. No extraction system extracts more than 61% of documents error-free. The strongest general-purpose coding agents, Claude Code Opus 5.5 and Codex GPT-6 Astra, outperform specialized extraction APIs on both perfect-document rate and Value F1, but at a higher cost per page. Among specialized extraction APIs, LlamaExtract spans the lower-cost frontier, with Agentic Plus Max Effort approaching the strongest coding agent on both perfect-document rate and Value F1 at lower cost per page. Our analysis of coding agent traces identifies intelligent image processing and programmatic reasoning, but also failures in applying document-specific definitions and recovering relationships from diagrams. We release ExtractBench Pro and these evaluation results as resources for the future development of improved frontier extraction systems.

==> figures/diagram_style.tex <==
\definecolor{mvInk}{HTML}{1E2530}%
\definecolor{mvMuted}{HTML}{5F6B7A}%
\definecolor{mvLine}{HTML}{BCC4CF}%
\definecolor{mvPanel}{HTML}{F4F6F9}%
\definecolor{mvBlue}{HTML}{2F6DB5}%
\definecolor{mvBlueFill}{HTML}{EAF2FB}%
\definecolor{mvOrange}{HTML}{CC5F06}%
\definecolor{mvOrangeFill}{HTML}{FDE9D3}%
\newcommand{\mvF}{\fontfamily{phv}\fontseries{m}\fontsize{6.4}{6.4}\selectfont}%
\newcommand{\mvS}[1]{\fontfamily{phv}\fontseries{m}\fontsize{#1}{#1}\selectfont\vphantom{Ag}}%
\newcommand{\mvB}[1]{\fontfamily{phv}\fontseries{b}\fontsize{#1}{#1}\selectfont\vphantom{Ag}}%
\newcommand{\mvT}{\fontfamily{lmtt}\fontseries{m}\fontsize{6.2}{6.2}\selectfont\vphantom{Ag}}%
\newcommand{\mvTB}{\fontfamily{lmtt}\fontseries{b}\fontsize{6.2}{6.2}\selectfont\vphantom{Ag}}%
\newcommand{\mvq}{\textquotedbl}%
\frenchspacing%
\tikzset{
  mv picture/.style={x=1pt,y=-1pt,
    every node/.style={inner sep=0pt,outer sep=0pt,text=mvInk,font=\mvF,execute at begin node=\vphantom{Ag}}},
  card/.style={draw=mvLine,line width=0.4pt,rounded corners=2pt,fill=white},
  tip/.style={-{Stealth[length=3.6pt,width=3.2pt]}},
  small tip/.style={-{Stealth[length=2.6pt,width=2.4pt]}},
  flow/.style={draw=mvInk,line width=0.6pt,tip},
  data/.style={draw=mvOrange,line width=0.8pt,tip},
  dev/.style={draw=mvBlue,line width=0.7pt,tip},
  loop/.style={dev,dash pattern=on 2.4pt off 1.6pt},
  knob/.style={draw=mvMuted,line width=0.5pt},
  place/.style={draw=mvMuted,line width=0.4pt,small tip}}%

